Context-Aware Prompt Tuning for Vision-Language Model with Dual-Alignment

Large-scale vision-language models (VLMs), e.g., CLIP, learn broad visual concepts from tedious training data, showing superb generalization ability. Amount of prompt learning methods have been proposed to efficiently adapt the VLMs to downstream tasks with only a few training samples. We introduce a novel method to improve the prompt learning of vision-language models by incorporating pre-trained large language models (LLMs), called Dual-Aligned Prompt Tuning (DuAl-PT). Learnable prompts, like CoOp, implicitly model the context through end-to-end training, which are difficult to control and interpret. While explicit context descriptions generated by LLMs, like GPT-3, can be directly used for zero-shot classification, such prompts are overly relying on LLMs and still underexplored in few-shot domains. With DuAl-PT, we propose to learn more context-aware prompts, benefiting from both explicit and implicit context modeling. To achieve this, we introduce a pre-trained LLM to generate context descriptions, and we encourage the prompts to learn from the LLM's knowledge by alignment, as well as the alignment between prompts and local image features. Empirically, DuAl-PT achieves superior performance on 11 downstream datasets on few-shot recognition and base-to-new generalization. Hopefully, DuAl-PT can serve as a strong baseline. Code will be available.

==> figs/method.tex <==
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.58\linewidth}
    % \vspace{0.6cm}
    \includegraphics[width=\linewidth]{figs/aaai-method-1 (7).pdf}
    \end{minipage}
    \begin{minipage}{0.34\linewidth}
        %\resizebox{0.8\linewidth}{!}{
        \begin{algorithm}[H]
            \caption{Solve Assignment Matrix.}
            \label{alg}            
            \begin{algorithmic}[1]
            %\resizebox{!}{0.8\linewidth}{
                \Require Local feature $\{\mathbf{z}_i\}_{i=1}^N$,prompts $\{\mathbf{w}\}_{i=1}^M$, vector $\mathbf{p},\mathbf{q}$, regularization $\lambda$
                %\State Compute cost for node match
                \State $\mathbf{C}_{WD} = 1 - \cos(\mathbf{Z},\mathbf{W})$
                %\State Compute intra-similarities 
                \State $\mathbf{C}_{z} = \cos{(\mathbf{Z},\mathbf{Z})}, \mathbf{C}_{w} = \cos{(\mathbf{W},\mathbf{W})}$ 
                \State $\mathbf{C}_{zw} = \mathbf{C}_z^2\mathbf{p}\mathbf{1}_M^\top + \mathbf{1}_N\mathbf{q}(\mathbf{C}_w^2)^\top$ 
                \For{$i=1,2,3,\cdots$}
                %\State Compute pseudo-cost matrix for GWD
                \State $\mathbf{C}_{GWD} = \mathbf{C}_{zw} - 2\mathbf{C}_z\mathbf{T}\mathbf{C}_w^\top$ 
                %\State Combine WD and GWD
                \State $\mathbf{C}_{graph} = \alpha \mathbf{C}_{GWD} + (1-\alpha)\mathbf{C}_{WD}$ 
                %\State Apply Sinkhorn to solve $\mathbf{T}$ with $\mathbf{C}_{graph}$
                \State $\mathbf{a} = \mathbf{1}, \mathbf{K} = \exp{(-\mathbf{C}_{graph}/\lambda)}$ 
                \For{$j=1,2,3,\cdots$}
                \State $\mathbf{a} = \mathbf{p}/\mathbf{Kb}, \mathbf{b} = \mathbf{q}/\mathbf{K}^\top\mathbf{a}$
                \EndFor
                \State $\mathbf{T} = \text{diag}(\mathbf{a})\mathbf{K}\text{diag}(\mathbf{b})$
                \EndFor
                %\Ensure Assignment Matrix $\mathbf{T}$
            \end{algorithmic}
        \end{algorithm}
    \end{minipage} 
    \caption{The illustration of the proposed method. The prompts are trained in a dual-alignment strategy, with the objective of learning from both the LLM and local images features.}
    \label{fig:minipage-with-algorithm}
\end{figure*}


==> tables/ab.tex <==
\begin{table*}[]
\centering

%\caption{Ablation study on other alternatives on few-shot recognition tasks. For feature selection, \textbf{CAM w/o noise}: only use CAM to select topK feature tokens; \textbf{Attention score}: select topK features according to the similarity with global token; \textbf{-}: use all the feature tokens without selection. For the alignment between local visual features and local prompts, \textbf{Graph}: our proposed graph match; \textbf{Attention}: use cross-attention to generate a dense alignment. }
\caption{Ablation studies on other alternatives on few-shot recognition tasks. For Feature selection, \textbf{None:} Do not perform feature selection during training; \textbf{TopK Sim}: Sample topK features according to similarity to global feature; \textbf{CAM Sample(+):} Also perform feature selection during inference; \textbf{CAM Sample:} Our proposed selection method. For cross-domain alignment, \textbf{Attention:} Apply cross-attention to match prompts with local features; \textbf{Node:} Only align node; \textbf{Edge:} Only align edge; \textbf{Graph:} Our proposed graph match. }
\label{table:analysis}
\begin{tabular}{cccccccc}
\toprule
Dataset                         & Feature Selection                     & Alignment                         & Shot-1                        & Shot-2                        & Shot-4                        & Shot-8                        & Shot-16                       \\ \hline
                                & \cellcolor[HTML]{ECF4FF}None          & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}19.00 & \cellcolor[HTML]{ECF4FF}19.27 & \cellcolor[HTML]{ECF4FF}22.17 & \cellcolor[HTML]{ECF4FF}26.40 & \cellcolor[HTML]{ECF4FF}31.77 \\
                                %& \cellcolor[HTML]{ECF4FF}TopK CAM      & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}18.10 & \cellcolor[HTML]{ECF4FF}19.17 & \cellcolor[HTML]{ECF4FF}23.30 & \cellcolor[HTML]{ECF4FF}26.57 & \cellcolor[HTML]{ECF4FF}31.97 \\
                                & \cellcolor[HTML]{ECF4FF}TopK Sim      & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}18.33 & \cellcolor[HTML]{ECF4FF}19.40 & \cellcolor[HTML]{ECF4FF}22.07 & \cellcolor[HTML]{ECF4FF}26.33 & \cellcolor[HTML]{ECF4FF}31.30 \\
                                & \cellcolor[HTML]{ECF4FF}CAM Sample(+) & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}18.70 & \cellcolor[HTML]{ECF4FF}19.36 & \cellcolor[HTML]{ECF4FF}22.63 & \cellcolor[HTML]{ECF4FF}26.67 & \cellcolor[HTML]{ECF4FF}31.37 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Attention & \cellcolor[HTML]{FFFFC7}16.23 & \cellcolor[HTML]{FFFFC7}18.03 & \cellcolor[HTML]{FFFFC7}22.00 & \cellcolor[HTML]{FFFFC7}26.07 & \cellcolor[HTML]{FFFFC7}31.40 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Node      & \cellcolor[HTML]{FFFFC7}19.07 & \cellcolor[HTML]{FFFFC7}19.03 & \cellcolor[HTML]{FFFFC7}22.50 & \cellcolor[HTML]{FFFFC7}26.67 & \cellcolor[HTML]{FFFFC7}31.77 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Edge      & \cellcolor[HTML]{FFFFC7}17.80 & \cellcolor[HTML]{FFFFC7}20.20 & \cellcolor[HTML]{FFFFC7}21.83 & \cellcolor[HTML]{FFFFC7}26.77 & \cellcolor[HTML]{FFFFC7}30.97 \\
\multirow{-7}{*}{FGVC Aircraft} & \cellcolor[HTML]{C9F8C8}CAM Sample    & \cellcolor[HTML]{C9F8C8}Graph     & \cellcolor[HTML]{C9F8C8}19.43 & \cellcolor[HTML]{C9F8C8}19.50 & \cellcolor[HTML]{C9F8C8}22.87 & \cellcolor[HTML]{C9F8C8}26.80 & \cellcolor[HTML]{C9F8C8}31.97 \\ \hline
                                & \cellcolor[HTML]{ECF4FF}None          & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}57.33 & \cellcolor[HTML]{ECF4FF}62.00 & \cellcolor[HTML]{ECF4FF}69.63 & \cellcolor[HTML]{ECF4FF}77.27 & \cellcolor[HTML]{ECF4FF}84.33 \\
                                %& \cellcolor[HTML]{ECF4FF}TopK CAM      & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}56.53 & \cellcolor[HTML]{ECF4FF}61.67 & \cellcolor[HTML]{ECF4FF}70.03 & \cellcolor[HTML]{ECF4FF}76.30 & \cellcolor[HTML]{ECF4FF}84.07 \\
                                & \cellcolor[HTML]{ECF4FF}TopK Sim      & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}54.90 & \cellcolor[HTML]{ECF4FF}62.17 & \cellcolor[HTML]{ECF4FF}69.00 & \cellcolor[HTML]{ECF4FF}77.20 & \cellcolor[HTML]{ECF4FF}84.63 \\
                                & \cellcolor[HTML]{ECF4FF}CAM Sample(+) & \cellcolor[HTML]{ECF4FF}Graph     & \cellcolor[HTML]{ECF4FF}56.10 & \cellcolor[HTML]{ECF4FF}60.57 & \cellcolor[HTML]{ECF4FF}70.17 & \cellcolor[HTML]{ECF4FF}77.30 & \cellcolor[HTML]{ECF4FF}84.37 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Attention & \cellcolor[HTML]{FFFFC7}52.40 & \cellcolor[HTML]{FFFFC7}60.70 & \cellcolor[HTML]{FFFFC7}70.03 & \cellcolor[HTML]{FFFFC7}76.53 & \cellcolor[HTML]{FFFFC7}83.10 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Node      & \cellcolor[HTML]{FFFFC7}57.10 & \cellcolor[HTML]{FFFFC7}62.10 & \cellcolor[HTML]{FFFFC7}70.47 & \cellcolor[HTML]{FFFFC7}77.23 & \cellcolor[HTML]{FFFFC7}84.50 \\
                                & \cellcolor[HTML]{FFFFC7}CAM Sample    & \cellcolor[HTML]{FFFFC7}Edge      & \cellcolor[HTML]{FFFFC7}52.47 & \cellcolor[HTML]{FFFFC7}62.47 & \cellcolor[HTML]{FFFFC7}70.57 & \cellcolor[HTML]{FFFFC7}77.60 & \cellcolor[HTML]{FFFFC7}84.60 \\
\multirow{-7}{*}{Euro SAT}      & \cellcolor[HTML]{C9F8C8}CAM Sample    & \cellcolor[HTML]{C9F8C8}Graph     & \cellcolor[HTML]{C9F8C8}58.37 & \cellcolor[HTML]{C9F8C8}63.43 & \cellcolor[HTML]{C9F8C8}70.20 & \cellcolor[HTML]{C9F8C8}77.43 & \cellcolor[HTML]{C9F8C8}84.67\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/ab2.tex <==
\begin{table*}[]
\centering

%\caption{Ablation study on other alternatives on few-shot recognition tasks. For feature selection, \textbf{CAM w/o noise}: only use CAM to select topK feature tokens; \textbf{Attention score}: select topK features according to the similarity with global token; \textbf{-}: use all the feature tokens without selection. For the alignment between local visual features and local prompts, \textbf{Graph}: our proposed graph match; \textbf{Attention}: use cross-attention to generate a dense alignment. }
\caption{Ablation studies on other alternatives on few-shot recognition tasks. For Feature selection, \textbf{None:} Do not perform feature selection during training; \textbf{TopK CAM}: Sample topK features according to CAM weights; \textbf{TopK Sim}: Sample topK features according to similarity to global feature; \textbf{CAM Sample(+):} Also perform feature selection during inference; \textbf{CAM Sample:} Our proposed selection method. For cross-domain alignment, \textbf{Attention:} Apply cross-attention to match prompts with local features; \textbf{Node:} Only align node; \textbf{Edge:} Only align edge; \textbf{Graph:} Our proposed graph match. }
\label{table:analysis}
\begin{tabular}{cccccccc}
\toprule
Dataset                         & Feature Selection                  & Alignment                     & Shot-1                        & Shot-2                        & Shot-4                        & Shot-8                        & Shot-16                       \\ \hline
                                & None                               & Graph                         & 19.00                         & 19.27                         & 22.17                         & 26.40                         & 31.77                         \\
                                    & TopK CAM                           & Graph                         & 18.10                         & 19.17                         & 23.30                         & 26.57                         & 31.97                         \\
                                & TopK Sim                           & Graph                         & 18.33                         & 19.40                         & 22.07                         & 26.33                         & 31.30                         \\
                                & CAM Sample(+)                      & Graph                         & 18.70                         & 19.36                         & 22.63                         & 26.67                         & 31.37                         \\ \cline{2-8}
                                & CAM Sample                         & Attention                     & 16.23                         & 18.03                         & 22.00                         & 26.07                         & 31.40                         \\
                                & CAM Sample                         & Node                          & 19.07                         & 19.03                         & 22.50                         & 26.67                         & 31.77                         \\
                                & CAM Sample                         & Edge                          & 17.80                         & 20.20                         & 21.83                         & 26.77                         & 30.97                         \\ \cline{2-8} 
\multirow{-8}{*}{FGVC Aircraft} & \cellcolor[HTML]{DEE0E3}CAM Sample & \cellcolor[HTML]{DEE0E3}Graph & \cellcolor[HTML]{DEE0E3}19.43 & \cellcolor[HTML]{DEE0E3}19.50 & \cellcolor[HTML]{DEE0E3}22.87 & \cellcolor[HTML]{DEE0E3}26.80 & \cellcolor[HTML]{DEE0E3}31.97 \\ \hline
                                & None                               & Graph                         & 57.33                         & 62.00                         & 69.63                         & 77.27                         & 84.33                         \\
                                & TopK CAM                           & Graph                         & 56.53                         & 61.67                         & 70.03                         & 76.30                         & 84.07                         \\
                                & TopK Sim                           & Graph                         & 54.90                         & 62.17                         & 69.00                         & 77.20                         & 84.63                         \\
                                & CAM Sample(+)                      & Graph                         & 56.10                         & 60.57                         & 70.17                         & 77.30                         & 84.37                         \\ \cline{2-8} 
                                & CAM Sample                         & Attention                     & 52.40                         & 60.70                         & 70.03                         & 76.53                         & 83.10                         \\
                                & CAM Sample                         & Node                          & 57.10                         & 62.10                         & 70.47                         & 77.23                         & 84.50                         \\
                                & CAM Sample                         & Edge                          & 52.47                         & 62.47                         & 70.57                         & 77.60                         & 84.60                         \\ \cline{2-8} 
\multirow{-8}{*}{Euro SAT}      & \cellcolor[HTML]{DEE0E3}CAM Sample & \cellcolor[HTML]{DEE0E3}Graph & \cellcolor[HTML]{DEE0E3}58.37 & \cellcolor[HTML]{DEE0E3}63.43 & \cellcolor[HTML]{DEE0E3}70.20 & \cellcolor[HTML]{DEE0E3}77.43 & \cellcolor[HTML]{DEE0E3}84.67\\
\bottomrule
\end{tabular}

\end{table*}

==> tables/ab_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\caption{\vspace{-0.3cm}Ablation Studies on 11 downstream datasets.}
\label{ab-table}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Feature Selection & Align & Shot1 & Shot2 & Shot4 & Shot8 & Shot16 \\ \hline
None              & Graph     & 61.88  & 63.30  & 67.02  & 70.32  & 73.84   \\
TopK CAM          & Graph     & 58.60  & 60.86  & 64.02  & 67.84  & 71.16   \\
TopK Sim          & Graph     & 62.09  & 63.57  & 66.95  & 70.73  & 74.06   \\
 
CAM Sample(+)     & Graph     & 62.23  & 63.47  & 67.18  & 70.41  & 74.00   \\ \hline
CAM Sample        & Attention & 58.87  & 60.70  & 65.15  & 68.49  & 72.44   \\
CAM Sample        & Node      & 62.10  & 63.38  & 67.28  & 70.35  & 73.97   \\
CAM Sample        & Edge      & 60.94  & 63.58  & 67.04  & 70.30  & 73.71   \\
\rowcolor[HTML]{DEE0E3} 
CAM Sample     & Graph     & 62.58  & 64.65  & 68.08  & 71.00  & 74.33  \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/dataset.tex <==
\begin{table}[h]
\centering
\caption{Detail of 11 downstream datasets.}
\label{supp:dataset}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Dataset      & Classes & Train & Val   & Test  & Task                       \\ \hline
ImageNet     & 1000    & 1.28M & N/A   & 50000 & generic-objects            \\
Caltech101   & 100     & 4128  & 1649  & 2465  & generic-objects            \\
OxfordPets   & 37      & 2944  & 736   & 3669  & fine-grained classifcation \\
StanfordCars & 196     & 6509  & 1635  & 8041  & fine-grained classifcation \\
Flowers102   & 102     & 4093  & 1633  & 2463  & fine-grained classifcation \\
Food101      & 101     & 50500 & 20200 & 30300 & fine-grained classifcation \\
FGVCAircraft & 100     & 3334  & 3333  & 3333  & fine-grained classifcation \\
SUN397       & 397     & 15880 & 3970  & 19850 & scene recognition          \\
DTD          & 47      & 2820  & 1128  & 1692  & texture                    \\
EuroSAT      & 10      & 13500 & 5400  & 8100  & satellite image            \\
UCF101       & 101     & 7639  & 1898  & 3783  & action recognition\\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/distill.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Ablation studies on different loss functions to distill from GPT. \textbf{WD}: Wasserstein Distance,
\textbf{CE}: Instance-wise cross-entropy, 
% working on the logits between learnable prompts and class description of each input sample. 
\textbf{Cosine}: Adopted cosine distance.}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{ccccccc}
\hline
Dataset                  & Loss       & Shot1          & Shot2          & Shot4         & Shot8          & Shot16         \\ \hline
\multirow{3}{*}{Caltech} & WD         & 89.50          & 90.27          & 90.87         & \textbf{91.63} & \textbf{92.50}          \\                       
                         & CE         & 87.37          & 89.27          & 90.27         & 90.27          & 91.00              \\
                         & Cosine     & \textbf{89.57} & \textbf{90.37} & \textbf{91.00}   & 91.33       & 92.43 \\ \hline
\multirow{3}{*}{DTD}     & WD         &47.03           &51.37           &54.83          &62.27           &\textbf{66.37}             \\
                         & CE         &45.23	          &49.63	       &53.83	        &60.00	            &63.70                \\
                         & Cosine     & \textbf{47.43} & \textbf{51.37} & \textbf{56.60} & \textbf{62.37} & 66.20  \\ \hline
\end{tabular}
}
\label{table:distill}
\end{table}
